Towards an Understanding of Default Policies in Multitask Policy Optimization

Much of the recent success of deep reinforcement learning has been driven by regularized policy optimization (RPO) algorithms with strong performance across multiple domains. In this family of methods, agents are trained to maximize cumulative reward while penalizing deviation in behavior from some reference, or default policy. In addition to empirical success, there is a strong theoretical foundation for understanding RPO methods applied to single tasks, with connections to natural gradient, trust region, and variational approaches. However, there is limited formal understanding of desirable properties for default policies in the multitask setting, an increasingly important domain as the field shifts towards training more generally capable agents. Here, we take a first step towards filling this gap by formally linking the quality of the default policy to its effect on optimization. Using these results, we then derive a principled RPO algorithm for multitask learning with strong performance guarantees.

==> m.macros.tex <==
\makeatletter

\newcommand{\define}[1]{{\bf #1}}
\newcommand{\figpanel}[1]{\textsf{#1}}
\newcommand{\todo}[1]{}
%\newcommand{\todo}[1]{[\textit{TODO: #1}]}

% some abbreviations

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}

\newcommand{\intinf}{\int_{-\infty}^{+\infty}}

% reference styles
\newcommand{\chpref}[1]{chapter~\ref{chp:#1}}
\newcommand{\Chpref}[1]{Chapter~\ref{chp:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[2]{figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\Figref}[2]{Figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\eqnref}[1]{(\ref{eqn:#1})}
\newcommand{\Eqnref}[1]{Equation (\ref{eqn:#1})}

% set horizontal margins to center text (using current paperwidth & textwidth)
\def\equalmargins{
	\setlength{\oddsidemargin}{\paperwidth}
	\addtolength{\oddsidemargin}{-\textwidth}
	\setlength{\oddsidemargin}{0.5 \oddsidemargin}
	\addtolength{\oddsidemargin}{-1in}
	\setlength{\evensidemargin}{\oddsidemargin}
}


% force equation numbers
\newenvironment{eqnforce}[1]{%
\let\savetheequation=\theequation% save the old equation number defn
\renewcommand{\theequation}{#1}%   set the equation string
\begin{equation}%		   start a normal equation env
}{%
\end{equation}%			   end it
\let\theequation=\savetheequation% restore the old defn
\addtocounter{equation}{-1}%       restore the counter which was incremented
}

% abbreviate \nonumber\\
\newcommand{\nn}{\nonumber\\}

% make text in super/subscripts the right size
\newcommand\mathbox[1]{\mathchoice{\mbox{#1}}{\mbox{#1}}%
{\mbox{\scriptsize{#1}}}{\mbox{\tiny{#1}}}}


% et al.
\newcommand{\etal}{\textit{et al$.$}}

% move the control point of the argument to the bottom of the box ...
\def\alignbottom#1{%
  \setbox0=\hbox{#1}%
  \raise\dp0\box0%
}
% ... or to the top ...
\newcommand{\aligntop}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=-\ht0%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}
% ... or to the middle.

\newcommand{\alignmiddle}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=\dp0%
  \advance\dimen0 by -\ht0%
  \divide\dimen0 by 2%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ tricks

\RequirePackage{tikz}

%% Create inline node: shorthand for \tikz[baseline,OPT1]{\node [OPT2] {ARG}}
%% some uses:
%% \tikznode[base]{foo}   
%% \tikznode[middle]{foo} 
%% \tikznode[below]{foo}
%% \tikznode[below=-1ex]{foo}
%% \tikznode[draw=red]{foo}       % tight red frame
%% \tikznode[framed=blue]{foo}    % adds some space (can be adjusted w/ inner sep
\newcommand\tikznode[1][]{%
  \@ifnextchar[{\m@tikznode[#1]}{\m@tikznode[][#1]}}
\def\m@tikznode[#1][#2]#3{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
  \tikz[baseline,#1]{\node [anchor=base,inner sep=0pt, #2] {#3};}%
  \endgroup%
}

%% Option to \path to annotate within a node (eg place text on a figure):
%% \node (fig) {\includegraphics{}};
%% \path[fit to node=fig] (0.1, 1) node {A};
\tikzoption{fit to node}{\tikzset{shift=(#1.south west), x=(#1.south east), y=(#1.north west)}}


%% Create inline node with pin label box pointing to content
%% \tikznodepin[env opts][inline node opts]{inline text}(pos)[pinnode
%% opts][pin edge opts]{pin text}

\tikzstyle{tikznode label node}=[]
\tikzstyle{tikznode label edge}=[->, very thick]
\tikzoption{tikznode label position}{#1\tikznodelabel@setposition#1}
\def\tikznodelabel@setposition(#1){\def\tikznodelabel@position{#1}}
\def\tikznodelabel@position{0, 5ex}

\def\tikznodelabel{%
  \@ifnextchar[{\tikznodelabel@m}{\tikznodelabel@@m[][]}
}
\def\tikznodelabel@m[#1]{%
  \@ifnextchar[{\tikznodelabel@@m[#1]}{\tikznodelabel@@m[][#1]}
}
\def\tikznodelabel@@m[#1][#2]#3{%
  \@ifnextchar({\tikznodelabel@@@m[#1][#2]{#3}}
               {\tikznodelabel@@@m[#1][#2]{#3}(\tikznodelabel@position)}
}
\def\tikznodelabel@@@m[#1][#2]#3(#4){%
  \@ifnextchar[{\tikznodelabel@@@@m[#1][#2]{#3}(#4)}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[][]}
}
\def\tikznodelabel@@@@m[#1][#2]#3(#4)[#5]{%
  \@ifnextchar[{\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5]}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5][]}
}
\def\tikznodelabel@@@@@m[#1][#2]#3(#4)[#5][#6]#7{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
%
  \tikz[baseline,#1]{
    \node (inl) [anchor=base,inner sep=0pt, #2] {#3};
    \useasboundingbox;
    \path (#4) node [tikznode label node, #5] {#7} 
               edge [tikznode label edge, #6] (inl);
   }%
  \endgroup%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parse a comma-separated list.  
%
% Latex provides \@for\var=first,second,...,last\do{code} which
% executes {code} many times, each time setting \var to the next item in
% the list 
% 
% This provides a variant \@forlast\var:=a,b,...,z\do{code}{codelast}
% which differs only on the last entry, for which it executes {codelast}.

\long\def\@forlast#1:=#2\do#3#4{%
  \expandafter\def\expandafter\@forlasttmp\expandafter{#2}%
  \ifx\@forlasttmp\@empty%
  \else%
    \expandafter\@forlastloop#2,\@nil,\@nil\@@#1{#3}{#4}%
  \fi%
}

\long\def\@forlastloop#1,#2,#3\@@#4#5#6{%
  \def#4{#1}%
  \ifx #4\@nnil%
    % empty list -- do nothing
  \else%
    \ifx #2\@nil% check if single item
      #6% apply #6 to #1
    \else%
      #5% apply #5 to #1
      \@forlastloop#2,#3\@@#4{#5}{#6}
    \fi%
  \fi%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Grab this page from an image file.  Can be used for a background.
%%   This version works 

%\newcommand\pageimage[1]{%
%  \hspace{-\oddsidemargin}\hspace*{-1in}%
%  \vspace*{-\topmargin}\vspace*{-\headheight}\vspace*{-\headsep}\vspace*{-1in}%
%  \makebox[top,left](0,0)\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio}{#1}
%} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% panel sizes.  

\let\panelwidth\columnwidth
\let\panelheight\textheight


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% image resizing.  width and height give maxima in terms of
%%   columnwidth and textheight respectively.

\def\parsesize[#1,#2]{{#1\panelwidth}{#2\panelheight}}

%% column image is deprecates

\def\mycolumnimage[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}
\newcommand{\columnimage}[2][1,.98]{\mycolumnimage[#1][]{#2}}

\def\mycenterimage[#1,#2][#3]#4{%
  \begin{center}\mycolumnimage[#1,#2][#3]{#4}\end{center}}



\newcommand{\centerimage}[2][1,.98]{\mycenterimage[#1][]{#2}}

\def\myvcenterimage[#1,#2][#3]#4{%
  \vfill\mycenterimage[#1,#2][#3]{#4}\vfill}
\newcommand{\vcenterimage}[2][1,.98]{\myvcenterimage[#1][]{#2}}

\newcommand{\columnline}[2][1]{\hbox to #1\panelwidth{#2}}
\renewcommand{\centerline}[2][1]{\hbox to #1\panelwidth{\hfil #2 \hfil}}


\newcommand{\columnimagestack}[2][1,.98]{%
  \@forlast\n@xtimg:=#2\do%
     {\makebox(0,0)[lb]{\mycolumnimage[#1][]{\n@xtimg}}}%
     {\mycolumnimage[#1][]{\n@xtimg}}%
}

%% so is scaleimage

\def\ScaleImgTwoOpt[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}

\def\ScaleImgOneOpt[#1,#2]{%
  \@ifnextchar[%]
    {\ScaleImgTwoOpt[#1,#2]}%
    {\ScaleImgTwoOpt[#1,#2][]}%
}

\def\scaleimage{%
  \@ifnextchar[%]
    {\ScaleImgOneOpt}%
    {\ScaleImgOneOpt[1,1]}%
}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% beamer extensions
\@ifclassloaded{beamer}{

%% Beamer controlled underbrace.  
%% \underbraceon<spec>[prefix]{maintext}{subtext}
%%   - prefix should probably live outside the \alt anyway
\newcommand<>{\underbraceon}[3][]{%
  \alt#4{%
    {#1{\underset{#3}{\underset{\text{\upbracefill}}{#2}}}}
  }{
    {#1{\underset{\phantom{#3}}{\underset{\phantom{\text{\upbracefill}}}{#2}}}}
  }%
}

} % end if beamer



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pgf extensions

\def\pgfp@nelparsearg[#1,#2]{%
  \def\pgfp@nelwidth{#1\panelwidth}%
  \def\pgfp@nelheight{#2\panelheight}}

\newenvironment{pgfpanel}[1][1,.995]
  {\pgfp@nelparsearg[#1]
   \begin{pgfpicture}{0cm}{0cm}{\pgfp@nelwidth}{\pgfp@nelheight}
      \pgftranslateto{\pgfpoint{0cm}{\pgfp@nelheight}}
      \pgfsetxvec{\pgfpoint{\pgfp@nelwidth}{0cm}}
      \pgfsetyvec{\pgfpoint{0cm}{-\pgfp@nelheight}}}
  {\end{pgfpicture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these use pgf to place a box at an arbitrary spot and (second form)
%% draw an arrow to the current position

\newcommand\placebox[4][left,baseline]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfputat{\pgfpoint{#2}{#3}}{\pgfbox[#1]{#4}}
  \end{pgfpicture}%
}

\newcommand\arrowbox[4][{0cm}{0cm}]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfnodebox{text}[virtual]{\pgfpoint{#2}{#3}}{#4}{2pt}{2pt}
    \pgfnodecircle{origin}[virtual]{\pgfpoint#1}{0pt}
    \pgfsetlinewidth{.5mm}
    \pgfsetendarrow{\pgfarrowsingle}
    \pgfnodeconnline{text}{origin}
  \end{pgfpicture}
}




% \def\alignmiddle#1{%
%   \setbox0=\hbox{#1}%
%   \dimen0=\dp0%
%   \advance\dimen0 by -\ht0%
%   \divide\dimen0 by 2%
%   \raise\dimen0\box0%
% }


\makeatother


==> m.symbols.tex <==
\RequirePackage{ifthen}
\RequirePackage{mathtools}

% use | for math mode
%\catcode`\|=3

% pg theory
\newcommand{\J}{\mathcal{J}^{\star}_\lambda}
\newcommand{\Jz}{\mathcal{J}^{\alpha}_\lambda}
\newcommand{\Ju}{\mathcal{J}_\lambda}
\newcommand{\kl}{\mathrm{KL}}
\newcommand{\pitheta}{\pi_{\theta}(a|s)}
\newcommand{\pistar}{\pi^*(a|s)}
\newcommand{\piz}{\pi_0(a|s)}
\newcommand{\St}{\mathcal S}
\newcommand{\A}{\mathcal A}
\newcommand{\eqtext}[1]{\ensuremath{\stackrel{\text{#1}}{=}}}
\newcommand{\Dinf}{\left\| \frac{d_{\rho}^{\pi^\star} }{\mu}  \right \|_\infty}
\newcommand{\kappaA}{\kappa^\alpha_{\mathcal A}(s)}
\newcommand{\Unif}{\mathrm{U}}
\newcommand{\tv}{d_{\mathrm{TV}}}

% DRL
\newcommand{\Dq}{\stackrel{D}{=}}
\newcommand{\Dqdef}{\stackrel{D}{\coloneqq}}
\newcommand{\bellop}{\mathcal{T}}

% use textmode for a short minus sign
\newcommand{\tminus}{\text{\textendash}}

% symbols for probability distributions
\newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
\newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
\newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}
% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\lr]{x} -> \mathbb{E}_a \lr[ x \lr]
\makeatletter
\def\expect{\@ifnextchar[{\expect@}{\expect@@[][\lr]}}
\def\expect@[#1]{\@ifnextchar[{\expect@@[#1]}{\expect@@[#1][\lr]}}
\def\expect@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{E}\newlr#2[{#3}#2]}%
             {\mathbb{E}_{#1}\newlr#2[{#3}#2]}}
\def\var{\@ifnextchar[{\var@}{\var@@[][\lr]}}
\def\var@[#1]{\@ifnextchar[{\var@@[#1]}{\var@@[#1][\lr]}}
\def\var@@[#1][#2]#3{%
  \ifthenelse{\equal{#1}{}}%
             {\mathbb{V}\newlr#2[{#3}#2]}%
             {\mathbb{V}_{#1}\newlr#2[{#3}#2]}}
\makeatother
\newcommand{\angles}[2][\lr]{{\newlr #1\langle{#2}#1\rangle}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathcal{E}}{=}}
% likelihoods
\newcommand{\like}[2]{\ensuremath{{\cal L}_{#1}\left({#2}\right)}}
\newcommand{\loglike}[2]{\ensuremath{\ell_{#1}\left({#2}\right)}}
\newcommand{\eff}{\mathcal{F}}
% info theoretic
\newcommand{\entropy}[2][\lr]{\ensuremath{\textbf{\textsf{H}}%
                             {\newlr #1[{#2}#1]}}}
\def\mutualinfo[#1;#2]{\ensuremath{\textbf{\textsf{I}}[{#1};{#2}]}}
\newcommand{\KL}[3][\lr]{\ensuremath{\textbf{\textsf{KL}}%
                             {\newlr #1[{#2}\lrmid #1\|{#3}#1]}}}
\newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
\newcommand{\normal}[3][\lr]{\ensuremath{\newlr\mathcal{N}#1(#2,#3#1)}}

% fractions
\newcommand{\half}{\ensuremath{{1\over2}}}
\newcommand{\overN}{\ensuremath{{1\over N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}

% whitened quantities
\newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\setV}{\ensuremath{{\cal V}}}
\newcommand{\setX}{\ensuremath{{\cal X}}}
\newcommand{\setY}{\ensuremath{{\cal Y}}}
\newcommand{\setZ}{\ensuremath{{\cal Z}}}
\newcommand{\size}[1]{\ensuremath{\left\vert{#1}\right\vert}}

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
\renewcommand{\vec}[1]{\ensuremath{\mathchoice%
{\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
{\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
\newcommand{\norm}[2][\lr]{\ensuremath{\newlr#1\|#2#1\|}}
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\renewcommand{\det}[2][\lr]{\ensuremath{\newlr#1\vert{#2}#1\vert}}
\newcommand{\trace}[2][\lr]{\ensuremath{\newlr\mathsf{Tr}#1[{#2}#1]}}
\newcommand{\diag}[2][\lr]{\ensuremath{\newlr\mathbox{\textsf{diag}}#1[{#2}#1]}}


% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\newcommand{\intdx}[1][dx]{\int\!\!#1\,}

\newcounter{multintctr}
\newcommand{\mltint}[1][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \int}

\newcommand{\mltintdx}[2][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \intdx[#2]}

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturals}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
%\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}


% accents

% adapted from symbols-a4.pdf; optional args permit shortening at left
% and right ends
\makeatletter
\def\widebar{\@ifnextchar[{\widebar@}{\widebar@@[3][0]}}
\def\widebar@[#1]{\@ifnextchar[{\widebar@@[#1]}{\widebar@@[#1][0]}}
\def\widebar@@[#1][#2]#3{{}\mkern#1mu\mkern#2mu\overline{\mkern-#1mu#3\mkern-#2mu}}
\makeatother    
        

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}


\newboolean{inlr}
\newboolean{midlr}
\setboolean{inlr}{false}
\newcommand\newlr{\setboolean{inlr}{false}}

\newcommand\lr[1]{%
  \ifthenelse{\boolean{inlr}}%
    {\ifthenelse{\boolean{midlr}}%
      {\middle#1\setboolean{inlr}{true}}
      {\right#1}}%
    {\left#1\setboolean{inlr}{true}}}%
\newcommand\lrmid{%
  \ifthenelse{\boolean{inlr}}%
    {\setboolean{midlr}{true}}
    {}}%


